Tiled Multiplane Images for Practical 3D Photography

The task of synthesizing novel views from a single image has useful applications in virtual reality and mobile computing, and a number of approaches to the problem have been proposed in recent years. A Multiplane Image (MPI) estimates the scene as a stack of RGBA layers, and can model complex appearance effects, anti-alias depth errors and synthesize soft edges better than methods that use textured meshes or layered depth images. And unlike neural radiance fields, an MPI can be efficiently rendered on graphics hardware. However, MPIs are highly redundant and require a large number of depth layers to achieve plausible results. Based on the observation that the depth complexity in local image regions is lower than that over the entire image, we split an MPI into many small, tiled regions, each with only a few depth planes. We call this representation a Tiled Multiplane Image (TMPI). We propose a method for generating a TMPI with adaptive depth planes for single-view 3D photography in the wild. Our synthesized results are comparable to state-of-the-art single-view MPI methods while having lower computational overhead.

==> src/A1.architecture.tex <==


\section{Network Architectures}
Detailed architectural specifications of the CNNs used for non-local feature extraction $\Theta(\cdot)$, disparity warping $\Phi(\cdot)$ and MPI generation $\Psi(\cdot)$ are provided in Tables~\ref{table:network-arch-theta},~\ref{table:network-arch-phi} and ~\ref{table:network-arch-psi}. All three networks are based on a U-Net architecture with depths four, four and three respectively. 

\begin{table}[h!]
\begin{center}
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Non-Local Feature Extraction Network} \\
\midrule
Layer & \textbf{k} & \textbf{s} & \textbf{p} & \makecell{{Channels} \\[-0.1cm]{(in/out)}}& Input \\
\midrule
conv1-1 & 3 & 1 & 1 & 4/4 & $\image{D} \oplus \image{I}$\\
conv1-2 & 3 & 1 & 1 & 4/4 & conv1-1 \\
maxpool1-1 & 3 & 1 & 1 & 4/4 & conv1-2 \\

conv2-1 & 3 & 1 & 1 & 4/8 & maxpool1-1 \\
conv2-2 & 3 & 1 & 1 & 8/8 & conv2-1 \\
maxpool2-1 & 3 & 1 & 1 & 8/8 & conv2-2 \\

conv3-1 & 3 & 1 & 1 & 8/16 & maxpool2-1 \\
conv3-2 & 3 & 1 & 1 & 16/16 & conv3-1 \\
maxpool3-1 & 3 & 1 & 1 & 16/16 & conv3-2 \\

conv4-1 & 3 & 1 & 1 & 16/32 & maxpool3-1 \\
conv4-2 & 3 & 1 & 1 & 32/32 & conv4-1 \\

up5-1 & & & & 32/32 & conv4-2 \\
conv5-1 & 3 & 1 & 1 & 48/16 & conv3-2 $\oplus$ up5-1 \\
conv5-2 & 3 & 1 & 1 & 16/16 & conv5-1 \\

up6-1 & & & & 16/16 & conv5-2 \\
conv6-2 & 3 & 1 & 1 & 24/8 & conv2-2 $\oplus$ up6-1 \\
conv6-3 & 3 & 1 & 1 & 8/8 & conv6-2 \\

up7-1 & & & & 8/8 & conv6-3 \\
conv7-2 & 3 & 1 & 1 & 12/4 & conv1-2 $\oplus$ up7-1 \\
conv7-3 & 3 & 1 & 1 & 4/24 & conv7-2 \\
\bottomrule
\end{tabular}
\caption{Detailed architecture of the non-local feature extraction network $\Theta(\cdot)$~(Sec.~3.2, main paper); \textbf{k},~\textbf{s},~\textbf{p} are the kernel size, stride and padding, $\oplus$ denotes concatenation along the channel dimension, and ``up'' is $\times$2 bilinear up-sampling.  All convolutional layers except the last are followed by batch normalization and a ReLU activation.}
\label{table:network-arch-theta}
\end{center}
\end{table}

\section{Extended Results}
Additional results on the \textit{Spaces} and \textit{Tanks and Temple} dataset are presented in Figures~\ref{fig:results-a} and \ref{fig:results-b}. \textbf{Please see the supplementary video for 3D photography results.}

\begin{table}[h!]
\begin{center}
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Disparity Warping Network} \\
\midrule
Layer & \textbf{k} & \textbf{s} & \textbf{p} & \makecell{{Channels} \\[-0.1cm]{(in/out)}}& Input \\
\midrule
conv1-1 & 3 & 1 & 1 & 28/32 & $\image{I}^i \oplus \image{D}^i \oplus \image{F}^i$\\
conv1-2 & 3 & 1 & 1 & 32/32 & conv1-1 \\
maxpool1-1 & 3 & 1 & 1 & 32/32 & conv1-2 \\

conv2-1 & 3 & 1 & 1 & 32/64 & maxpool1-1 \\
conv2-2 & 3 & 1 & 1 & 64/64 & conv2-1 \\
maxpool2-1 & 3 & 1 & 1 & 64/64 & conv2-2 \\

conv3-1 & 3 & 1 & 1 & 64/128 & maxpool2-1 \\
conv3-2 & 3 & 1 & 1 & 128/128 & conv3-1 \\
maxpool3-1 & 3 & 1 & 1 & 128/128 & conv3-2 \\

conv4-1 & 3 & 1 & 1 & 128/256 & maxpool3-1 \\
conv4-2 & 3 & 1 & 1 & 256/256 & conv4-1 \\

up5-1 & & & & 256/256 & conv4-2 \\
conv5-1 & 3 & 1 & 1 & 384/128 & conv3-2 $\oplus$ up5-1 \\
conv5-2 & 3 & 1 & 1 & 128/128 & conv5-1 \\

up6-1 & & & & 128/128 & conv5-2 \\
conv6-2 & 3 & 1 & 1 & 192/64 & conv2-2 $\oplus$ up6-1 \\
conv6-3 & 3 & 1 & 1 & 64/64 & conv6-2 \\

up7-1 & & & & 64/64 & conv6-3 \\
conv7-2 & 3 & 1 & 1 & 96/32 & conv1-2 $\oplus$ up7-1 \\
conv7-3 & 3 & 1 & 1 & 32/1 & conv7-2 \\
\bottomrule
\end{tabular}
\caption{Detailed architecture of the disparity network $\Phi(\cdot)$ used for per-tile MPI plane prediction~(Sec.~3.2, main paper); \textbf{k},~\textbf{s},~\textbf{p} are the kernel size, stride and padding, $\oplus$ denotes concatenation along the channel dimension, and ``up'' is $\times$2 bilinear up-sampling.  All convolutional layers except the last are followed by a ReLU activation and batch normalization. The last layer has a sigmoid activation. }
\label{table:network-arch-phi}
\end{center}
\end{table}


\begin{table}[h!]
\setlength{\tabcolsep}{6pt}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{MPI Generation Network} \\
\midrule
Layer & \textbf{k} & \textbf{s} & \textbf{p} & \makecell{{Channels} \\[-0.1cm]{(in/out)}}& Input \\
\midrule
conv1-1 & 3 & 1 & 1 & (28 + $n$)/32 & 
%\makecell{{$\image{I}^i \oplus \image{D}^i \oplus$} \\[-0.1cm]{$\image{F}^i \oplus \{ {M}^i_k \}$)}} \\
$\image{I}^i \oplus \image{D}^i \oplus \image{F}^i \oplus \{ {M}^i_k \}$\\
conv1-2 & 3 & 1 & 1 & 32/32 & conv1-1 \\
maxpool1-1 & 3 & 1 & 1 & 32/32 & conv1-2 \\

conv2-1 & 3 & 1 & 1 & 32/64 & maxpool1-1 \\
conv2-2 & 3 & 1 & 1 & 64/64 & conv2-1 \\
maxpool2-1 & 3 & 1 & 1 & 64/64 & conv2-2 \\

conv3-1 & 3 & 1 & 1 & 64/128 & maxpool2-1 \\
conv3-2 & 3 & 1 & 1 & 128/128 & conv3-1 \\

up4-1 & & & & 128/128 & conv3-2 \\
conv4-1 & 3 & 1 & 1 & 192/64 & conv2-2 $\oplus$ up4-1 \\
conv4-2 & 3 & 1 & 1 & 64/64 & conv4-1 \\

up5-1 & & & & 64/64 & conv4-2 \\
conv5-2 & 3 & 1 & 1 & 96/32 & conv1-2 $\oplus$ up5-1 \\
conv5-3 & 3 & 1 & 1 & 32/($n - 1 + 3)$  & conv5-2 \\
\bottomrule
\end{tabular}
}
\caption{Detailed architecture of the MPI generation network $\Psi(\cdot)$ with $n$ planes per tile~(Sec.~3.2, main paper); \textbf{k},~\textbf{s},~\textbf{p} are the kernel size, stride and padding, $\oplus$ denotes concatenation along the channel dimension, and ``up'' is $\times$2 bilinear up-sampling.  All convolutional layers except the last are followed by a ReLU activation and batch normalization. The last layer has a sigmoid activation. The output is $n-1$ alpha layers and a single background RGB. }
\label{table:network-arch-psi}
\end{center}
\end{table}



==> src/A2.results.tex <==


\begin{figure*}[t!]
  \centering
   \includegraphics[width=1.0\linewidth, trim={0cm, 10cm, 0cm, 0cm}, clip]{images/supp-graph.pdf}
   \caption{Quantitative evaluation of the effect of tile size and number of planes on novel view synthesis quality. In general, a small number of planes and a small tile size provide better results.}
   \label{fig:tiles-planes}
\end{figure*}

\section{Tile Size \& Number of Depth Planes}
Figure~\ref{fig:tiles-planes} evaluates the effect of tile size and number of planes on the quality of novel view synthesis. For four and eight planes per tile, increasing the tile size lowers quality overall.  This supports the observation --- and the motivation for tiled multiplane images --- that the local depth complexity of a scene is low, and can be adequately represented with a small number of MPI planes. But, as observed, this fails to hold true as the size of the local region increases. For sixteen planes, on the other hand, the quality is improved as the tile size increases. Furthermore, increasing the number of depth planes for a fixed tile size lowers performance in general. This agrees with the observations of Khakhulin~\etal~\cite{khakhulin2022} and Hu~\etal~\cite{hu2021} that reductive models are unable to handle redundant geometry effectively. Moreover, the  model's complexity increases proportionately with the number of depth planes, leading to slower convergence and higher error for the same number of training steps.

\begin{figure*}[h!]
   \includegraphics[width=1.0\linewidth, trim={0cm, 0cm, 18.0cm, 0cm}, clip]{images/results-supp-a.pdf}
\caption{Qualitative comparison of the novel view synthesis results of the baseline methods and our approach on the \emph{Spaces} dataset. Our results are comparable to AdaMPI, and much sharper than SVMPI, VMPI and MINE.  }
\label{fig:results-a}
\vspace{-3mm}
\end{figure*}

\begin{figure*}[h!]
   \includegraphics[width=1.0\linewidth, trim={0cm, 0cm, 18.0cm, 0cm}, clip]{images/results-supp-b.pdf}
\caption{Further results on the \emph{Spaces} and \emph{Tanks and Temples} dataset.   }
\label{fig:results-b}
\vspace{-3mm}
\end{figure*}
